NLLG Quarterly arXiv Report 09/23: What are the most influential current AI Papers?

Artificial Intelligence (AI) has witnessed rapid growth, especially in the subfields Natural Language Processing (NLP), Machine Learning (ML) and Computer Vision (CV). Keeping pace with this rapid progress poses a considerable challenge for researchers and professionals in the field. In this arXiv report, the second of its kind, which covers the period from January to September 2023, we aim to provide insights and analysis that help navigate these dynamic areas of AI. We accomplish this by 1) identifying the top-40 most cited papers from arXiv in the given period, comparing the current top-40 papers to the previous report, which covered the period January to June; 2) analyzing dataset characteristics and keyword popularity; 3) examining the global sectoral distribution of institutions to reveal differences in engagement across geographical areas. Our findings highlight the continued dominance of NLP: while only 16% of all submitted papers have NLP as primary category (more than 25% have CV and ML as primary category), 50% of the most cited papers have NLP as primary category, 90% of which target LLMs. Additionally, we show that i) the US dominates among both top-40 and top-9k papers, followed by China; ii) Europe clearly lags behind and is hardly represented in the top-40 most cited papers; iii) US industry is largely overrepresented in the top-40 most influential papers.

==> structure/0201_someotherstuff.tex <==
\subsection*{Analysis} 




\iffalse
\begin{figure}[H] % Exemplo de imagem
					\vspace*{-1cm}
					\includegraphics[width=\linewidth]{regression.png}
\end{figure}
\vspace{0.5cm}
\fi 




\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_citation_counts_by_week_all (3).png}
    \caption{Weekly Mean Citation for papers in the last 7 months}
    \label{fig:}
\end{figure}



%Surprisingly, the LG category appears to be underrepresented in terms of citation counts.
%On the other hand, the CL category exhibits higher citation counts on average, particularly at the beginning of the year, indicating a strong presence and popularity of papers in this domain. Although some papers were categorized under both AI and LG, we focused primarily on their primary category to ensure a more focused representation.
%\todo{SE: check this}
%\vspace{1cm}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_count_categories_count.png}
    \caption{Weekly overview of number of papers published in the last 7 months by category}
    \label{fig:}
\end{figure}



%\vspace{1cm}






Based on the figures and analysis, it is evident that the terms "ChatGPT" and "LLMs" show a more pronounced presence in the titles and abstracts of papers within the cs.AI category compared to cs.LG. However, both cs.AI and cs.LG categories exhibit a lower rate of appearance of these terms when compared to the cs.CL category.

The cs.CL category demonstrates a notable increase and subsequent decrease in the occurrence of the terms over time, indicating a stronger correlation with the publication of papers and mean citation counts compared to the other categories.

On the other hand, while cs.AI shows a relatively higher presence of the terms, it does  follow the same significant pattern of increase and decrease as in cs.CL. Similarly, cs.LG shows even lower rates of appearance of the terms and lacks a clear pattern of increase and decrease over time.

These observations suggest that cs.AI has a relatively higher association with the terms "ChatGPT" and "LLMs" compared to cs.LG, but both categories exhibit lower rates of term occurrence when compared to cs.CL. Further investigation is needed to understand the underlying reasons behind these differences and their potential impact on the publication dynamics and citation means within each specific category.

\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=0.5\linewidth]{structure/pics/terms_chatgpt (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_llm (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_llama (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_only_categories_chatGPT.pdf}
    \caption{Terms in title and abstract for all papers. Top left: ``GPT'', top right: ``LLMs''. Bottom left: ``LLAMA''. Bottom right: ``ChatGPT''.}
    \label{fig:}
\end{figure}
%\vspace{1cm}

%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_llm (1).pdf}
%    \caption{Terms LLMs in title and abstract for all papers}
%    \label{fig:}
%\end{figure}

%\vspace{1cm}

%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_llama (1).pdf}
%    \caption{Terms LLAMA in title and summary for all papers}
%    \label{fig:}
%\end{figure}
%plot terms by category
%\vspace{1cm}
%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_only_categories_chatGPT.pdf}
%    \caption{Terms chatGPT in title and summary for papers  filtered  by the 3  categories}
%    \label{fig:}
%\end{figure}
%\vspace{1cm}
%
%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics%/terms_only_categories_llm.pdf}
%    \caption{Terms LLM in title and summary for papers filtered  by the 3  categories}
%    \label{fig:}
%\end{figure}

%\vspace{1cm}
\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/terms_only_categories_llama (1).pdf}
    \caption{Terms LLAMA in title and summary for papers  filtered  by the 3  categories}
    \label{fig:}
\end{figure}

Based on the figures and analysis, we can observe a clear pattern in the occurrence of the terms "ChatGPT" and "LLMs" within the titles and abstracts of the papers. In the case of category cs.CL, there is a notable increase and subsequent decrease in the appearance of these terms over time, alongside a corresponding trend in the publication of papers and mean citation counts. This indicates a potential relationship between the terms' prevalence, paper publication, and citation counts within the cs.CL category. The other categories, cs.LG and cs.AI, also show distinctive patterns, suggesting different trends in term usage, paper publication, and citation means within each specific category.


\vspace{1cm}


\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/terms_by_category (1).png}
    \caption{Terms gpt or LLMs in title and summary by category}
    \label{fig:}
\end{figure}




%\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/papers_published_by_timeWeek_all.png}
 %   \caption{Weekly overview of number of papers published in the last 7 months}
  %  \label{fig:}
%\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/papers_published_by_time_all_Month.pdf}
    \caption{Overall number of papers published in the last 7 months}
    \label{fig:}
\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_count_categories_sorted_month.pdf}
    \caption{Overall number of papers published in the last 7 months}
    \label{fig:}
\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/papers_over_time_until_july.pdf}
    \caption{Number of Papers published in the last 7 months by different categories}
    \label{fig:}
\end{figure}

==> structure/99_limitations.tex <==
\section*{Limitations}\label{limitation}
Limitations of our approach include the following. First of all, the discrepancy of citation counts from different tools such as SemanticScholar or GoogleScholar still exists. In our last report, LLaMA has 874 citations according to SemanticScholar (July 29, 2023) but only 710 citations according to GoogleScholar with a relative difference of $\frac{164}{874} = 18.7\%$. 
This time we observe 1891 from GoogleScholar (November 7, 2023) and  2372 from SemanticScholar (November 7, 2023)  with a difference of 20.3\%.  
The paper with the fewest citations in our top-20 list \cite{yang2023large} has 36 citations (November 7, 2023) according to SemanticScholar but 29 citations according to GoogleScholar, a relative difference of $\frac{7}{36} = 19.4\%$. As discussed in the previous report, such (growing) deviations may bias our selection of papers. Secondly, focusing particularly on highly cited papers may induce a bias towards these papers similar to that of a self-fulfilling prophecy or preferential attachment. Thirdly, our focus on weekly citation averages may have unexpected effects: for example, papers submitted in a week with fewer average citations may enjoy certain benefits and end up ranking higher than papers with more citations but are published in a competitive week with an average high citation counts; Another example is papers published on the verge of our analysis period may be unfairly punished due to the incomplete week decision. Finally, some authors and research groups, potentially more traditional ones, may refrain from submitting their papers to arXiv, despite its otherwise high popularity, particularly in the computer science community (see exponential submission growth rates of arXiv submission numbers in the last decades \url{https://info.arxiv.org/help/stats/2021_by_area/index.html}). Papers from such authors or groups will not be part of our dataset and analysis. 

Our limitations must be kept in mind when interpreting our results. 

\todo{SE: p.s. the appendix needs to be referenced in the main text}

%\todo{SE: new papers could also be highlighted in the main tables, not only the ones from July onwards. Maybe with a different highlighting technique?}
%\todo[zr]{Done}

==> structure/abstract_old.tex <==
\begin{abstract}
    The rapid growth of information in the field of Generative Artificial Intelligence (AI), particularly in the subfields of Natural Language Processing (NLP) and Machine Learning (ML), presents a significant challenge for researchers and practitioners to keep pace with the latest developments. To address the problem of information overload, this report by the Natural Language Learning Group at Bielefeld University focuses on identifying the most popular papers on arXiv, with a specific emphasis on NLP and ML. The objective is to offer a quick guide to the most relevant and widely discussed research, aiding both newcomers and established researchers in staying abreast of current trends.
%
%The report leverages the comprehensive and expeditious publication process of arXiv, a prominent pre-print repository, to 
In particular, we compile a list of the 40 most popular papers based on normalized citation counts from the first half of 2023. %Among our key findings, NLP emerges as more influential than ML in terms of citations, despite the presence of more ML papers in the dataset. Notably, 
We observe the dominance of papers related to Large Language Models (LLMs) and specifically ChatGPT during the first half of 2023, with the latter showing signs of declining popularity more recently, however. Further, NLP related papers are the most influential (around 60\% of top papers) even though there are twice as many ML related papers in our data. Core issues investigated in the most heavily cited papers are:  
%
%The investigation delves into various aspects, including 
LLM efficiency, evaluation techniques, ethical considerations, embodied agents, and problem-solving with LLMs. %indicating the focal points of current research interest. 
Additionally, we examine the characteristics of top papers in comparison to others outside the top-40 list (noticing the top paper's focus on LLM related issues and higher number of co-authors) and analyze the citation distributions in our dataset, among others. 
%and track the popularity of ChatGPT, a significant contributor to the recent LLM hype.
%
%The report aims to assist both newcomers and established researchers by providing accessible links to pertinent literature. Future plans include regular updates to observe evolving trends over time, deeper analysis of the arXiv dataset, and the inclusion of other AI-related arXiv categories (e.g., cs.CV, stat.ML, cs.AI). The open availability of code and data from this study contributes to the advancement of the field and fosters collaboration among researchers in the AI community.
\end{abstract}


==> structure/tables/VIF.tex <==
\begin{table}[H]
\fontsize{9pt}{9pt}\selectfont
\centering
\begin{tabular}{ll}
\hline
\textbf{Feature}  & \textbf{VIF}  \\
\hline
Publication month &	1.01 \\
\#Author &	1.01  \\
\hline
\end{tabular}
\caption{\label{apdx:vif_table}
Variance inflation factor for numerical features.}
\end{table}

==> structure/tables/author_avg.tex <==
\begin{table}[!htp]
\centering
\scriptsize
\begin{tabular}{lccc}\toprule
&\textbf{Industry} & \textbf{Academia} \\\midrule
\textbf{Independent Research }&18.6 & 9.3 \\
&\multicolumn{2}{c}{\textit{Collaboration}} \\
\textbf{-with Industry} &0 &- \\
\textbf{-with Academia} &16.9 &14.6 \\
\bottomrule
\end{tabular}
\caption{Average number of authors across authorship status in the top-40 papers.}
\label{tab:author}
\end{table}

==> structure/tables/nww_previous.tex <==
\begin{table}[H]
\fontsize{9pt}{9pt}\selectfont
\centering
\begin{tabular}{ccc}
\toprule
& \multicolumn{2}{l}{\#New papers (vs. previous report)} \\
\cmidrule{2-3}
&Jan.-June &July-Sept.  \\
\midrule
20 list  &3 &4\\
21-40 list  &6 &6 \\
\midrule
Total & 9 & 10 \\
\bottomrule
\end{tabular}
\caption{\label{table:old-new-previous}
\zr{New papers that appear in the Jan-Sept top-40 list (Tables \ref{table:top20} and \ref{table:top40}) compared to the Jan-June top-40 list from previous report \cite{eger2023nllg}. We list the number of new papers in the top-20 list and the 21-40 list, respectively. We split the count of papers by their publication time in columns \textit{Jan-June} and \textit{July-Sept}. } }
\end{table}

==> structure/tables/reg.tex <==
\begin{table}[!htbp]
\centering
\fontsize{9pt}{9pt}\selectfont
\begin{tabular}{cc:cccc} 
\hline
\multicolumn{2}{c:}{\textbf{Numerical}} & \multicolumn{4}{c}{\textbf{Categorical}} \\
 $\beta_{\text{Month}}$ & $\beta_{\#\text{Author}}$ &  $\beta_{\text{GPT}}$ & $\beta_{\text{LLM}}$ & $\beta_{\text{Llama}}$ & $\beta_{\text{Modal}}$\\
\hline
-0.533$^{***}$ & 0.652$^{***}$ & 7.524$^{***}$ & 2.498$^{***}$  & 24.6752$^{***}$  & 6.009$^{***}$\\
\hline
\end{tabular}
\caption{\label{reg:feature}
Regression results for paper features. The corresponding p-value is obtained through a two-tailed Student's t-test for coefficients at significance level 0.05 (*), 0.01 (**), 0.001 (***).}
\end{table} 

==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3b - 25/02/2019

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=Week,
  timeline width/.store in=\timelinewidth,
  timeline width=20,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.05,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}

\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  \draw[fill,opacity=0.8] (0,0) rectangle (\timelinewidth,\timelineheight);
  \shade[top color=black, bottom color=white,middle color=black!20]
    (0,0) rectangle (\timelinewidth,-\timelineoffset);
  \shade[top color=white, bottom color=black,middle color=black!20]  
    (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\tlmxi] in {#2}  {\global\let\maxsmitem\tlmxi}%
  \else%
    \foreach \smitem [count=\tlmxi] in {1,...,#2}  {\global\let\maxsmitem\tlmxi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\tlmxi] in {#2}{%
      \node[text=white,text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \else%
    \foreach \x[count=\tlmxi] in {1,...,#2}{%
      \node[text=white, text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels
% 0.3b -> \xi conflict - thanks Enrico Gregorio (egreg) https://tex.stackexchange.com/q/476089
